Relaxing the Assumptions of Knockoffs by Conditioning

The recent paper Cand\`es et al. (2018) introduced model-X knockoffs, a method for variable selection that provably and non-asymptotically controls the false discovery rate with no restrictions or assumptions on the dimensionality of the data or the conditional distribution of the response given the covariates. The one requirement for the procedure is that the covariate samples are drawn independently and identically from a precisely-known (but arbitrary) distribution. The present paper shows that the exact same guarantees can be made without knowing the covariate distribution fully, but instead knowing it only up to a parametric model with as many as $\Omega(n^{*}p)$ parameters, where $p$ is the dimension and $n^{*}$ is the number of covariate samples (which may exceed the usual sample size $n$ of labeled samples when unlabeled samples are also available). The key is to treat the covariates as if they are drawn conditionally on their observed value for a sufficient statistic of the model. Although this idea is simple, even in Gaussian models conditioning on a sufficient statistic leads to a distribution supported on a set of zero Lebesgue measure, requiring techniques from topological measure theory to establish valid algorithms. We demonstrate how to do this for three models of interest, with simulations showing the new approach remains powerful under the weaker assumptions.

==> appSeqGGM.tex <==

% not for sending the first draft.  
%\subsection{An Alternative Knockoff for Gaussian Graphical models}%TODO
This section provides an alternative construction for Gaussian graphical models \eqref{eq:gauss_sparse}. It also relies on the blocking idea in Algorithm~\ref{alg:sparse-gaussian-or}, but different from the latter in constructing the knockoff for each connected component in a sequential way rather than applying the low-dimensional construction. This sequential algorithm conditions on fewer statistics than Algorithm~\ref{alg:sparse-gaussian-or} and does not need to compute $\bss$. However, there is a gap in the proof of its validity which we decide to leave as a conjecture. 

\subsection{The Algorithm}
Algorithm~\ref{alg:sparse-gaussian} allows constructing knockoff columns in any order as $(\pi_1,\dots,\pi_p)$. For ease of discussion, in the text we take $\pi_j=j$. The set $N_j$ contains the \emph{neighbors} of $j$ in the sense that $\bXk_j$ is required to satisfy 
\begin{align}\label{eq:hdg-req}
\forall\; k\in N_j, 
\langle \bXk_j,\bX_k\rangle =\langle\bX_j,\bX_k\rangle \mbox{ , and if } k<j \mbox{ also }\langle\bXk_j,\bXk_k\rangle=\langle\bX_j,\bXk_k\rangle. 
\end{align}
$N_j$ is initialized as $I_j$ (line~\ref{line2}) but unfortunately to ensure swap exchangeability, it must expa`nd every time a knockoff column is generated for any variable in $N_j$ (line~\ref{line7}). The input integer $n'$ is upper-bounded by $n$ with default value $n$. At the $j$th step, if the size of $N_j$ is not too large relative to $n'$, we run Algorithm~\ref{alg:rotate-residual} to create a nontrivial knockoff for $\bX_j$ by sampling uniformly from all vectors that satisfy both \eqref{eq:hdg-req} and $\bs{1}_n\tp \bXk_j=\bs{1}_n\tp \bX_j$; otherwise $j$ is added to the \textit{blocking set} $B$. Except for the sampling step, Algorithm~\ref{alg:sparse-gaussian} is similar to Algorithm~\ref{alg:ggm-greedy-search} which searches a blocking set in Section~\ref{sec:eg-ggm}. 
 %, which is initialized as the input $B_0$ (default $\emptyset$), is 
 
%If the order $\pi$ is only partially given, say $(\pi_1,\dots, \pi_{j_0})$, Algorithm~\ref{alg:sparse-gaussian} can be modified accordingly: at the $j$th step for $j>j_0$, we assign $\pi_j$ to be the $k$ with smallest $|N_k|$ among $[p]\setminus  \{ \pi_{1},\dots,\pi_{j-1} \}$, with ties broken at random.

% Discussion on the algorithm
%Similar to $\bU$ in the previous section, the $\tbe_j$ in Algorithm~\ref{alg:eg-ggm} can be generated by a QR decomposition, plus a renormalization so that $\|\tbe_j\|=\|\be_j\|$, as long as $n\ge |I_j|+|I_j'|+2$. % complexity is O(n^3)
\begin{algorithm}[h]
\caption{Conditional Knockoffs for Gaussian Data with a Sparse Precision Matrix} \label{alg:sparse-gaussian}
%\algsetup{linenodelimiter=}
\begin{algorithmic}[1]
\STATE \textbf{Input}: $\bX$, $\pi$, $E$, $n'$($\leq n$, default $=n$). 
\STATE Initialize $N_j=I_j $ for all $j\in [p]$, $B=\emptyset$\label{line2}
\FOR{$j = 1,\dots,p$}
\STATE Let $N_j^{-}=N_j\cap \{\pi_1,\dots, \pi_{j-1} \} \setminus B$, and $N_j^{+}=N_j\setminus N_j^{-} $
\IF{$n' \geq 2+ |N_j|+|N_j^-|  $}
\STATE Create $\bXk_{\pi_j}$ by Algorithm~\ref{alg:rotate-residual} 
\begin{comment}
\STATE Compute $\hbb^{(j)}$ and $\tbb^{(j)}$ as the least-squares coefficient vectors from regressing $\bX_{\pi_j}-\hbmu_{\pi_j}$ on $\bX_{N_j}-\hbmu_{N_j}$ and $\bXk_{N_j^{-}} - \hbmu_{N_j^{-}}$. That is, 
\[\bX_{\pi_j}-\hbmu_{\pi_j} = \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j,\]
where $\left[\bs{1}_n,\, \left(\bX_{N_j}-\hbmu_{N_j}\right),\, \left( \bXk_{N_j^{-}}-\hbmu_{N_j^{-}} \right)\right]^\top\be_j = \bs{0}_{|N_j|+|N_j^{-}|+1}$.
\STATE Sample $\tbe_j$ uniformly (and conditionally independently of $\bX_j$) from the left null space of $\left[\bs{1}_n,\, \left(\bX_{N_j}-\hbmu_{N_j}\right),\, \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\right]$ with norm $\|\be_j\|$ and set
\[ \bXk_{\pi_j} = \hbmu_{\pi_j} + \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbe_j.\]
\end{comment}
\STATE Update $N_k\leftarrow N_k \cup ( N_j\setminus  \{k\})$ for all $k\in N_j^{+}$\label{line7}
\ELSE
\STATE $\bXk_{\pi_j}=\bX_{\pi_j}$
\STATE $B\leftarrow B\cup \{j\}$
\ENDIF
\ENDFOR
\RETURN $\bXk = [\bXk_1,\dots,\bXk_p]$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Subroutine: Residual Rotation } \label{alg:rotate-residual}
%\algsetup{linenodelimiter=}
\begin{algorithmic}[1]
\STATE Compute $\hbb^{(j)}$ and $\tbb^{(j)}$ as the least-squares coefficient vectors from regressing $\bX_{\pi_j}-\hbmu_{\pi_j}$ on $\bX_{N_j}-\hbmu_{N_j}$ and $\bXk_{N_j^{-}} - \hbmu_{N_j^{-}}$. That is, 
\[\bX_{\pi_j}-\hbmu_{\pi_j} = \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j,\]
where $\left[\bs{1}_n,\, \left(\bX_{N_j}-\hbmu_{N_j}\right),\, \left( \bXk_{N_j^{-}}-\hbmu_{N_j^{-}} \right)\right]^\top\be_j = \bs{0}_{|N_j|+|N_j^{-}|+1}$.
\STATE Sample $\tbe_j$ uniformly % (and conditionally independently of $\bX_j$) 
from the left null space of $\left[\bs{1}_n,\, \left(\bX_{N_j}-\hbmu_{N_j}\right),\, \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\right]$ with norm $\|\be_j\|$ and set
\[ \bXk_{\pi_j} = \hbmu_{\pi_j} + \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbe_j.\]
\end{algorithmic}
\end{algorithm}

The $\tbe_j$ in Algorithm~\ref{alg:rotate-residual} can be generated by regressing a $n$-dimension random vector with i.i.d. standard normal entries on the regressors, plus a renormalization so that $\|\tbe_j\|=\|\be_j\|$, as long as $n\ge |N_j|+|N_j^{-}|+2$. Such a construction ensures that $\bXk_j$ is different from $\bX_j$ and does not lie in any hyperplane spanned by some of $\bX_k$'s and $\bXk_k$'s almost surely.
%The computational complexity of Algorithm~\ref{alg:sparse-gaussian} will depend on the sparsity, both in its magnitude and pattern, but a simple upper-bound is given by \ljmargin{$O(n|I_{\text{max}}|^2p)$}{check}, where $I_{\text{max}}$ is a/the largest neighborhood.
%[Note: this sentence is not accurate]
%The computational complexity of Algorithm~\ref{alg:sparse-gaussian} depends on the sparsity, both in its magnitude and pattern, but a simple upper-bound is given by $O(n n'^{2} p)$. %, where $N_{\text{max}}$ is the largest $N_j$.
The computational complexity of Algorithm~\ref{alg:sparse-gaussian} has a simple upper-bound $O( p n n'^{2} )$ since each regression takes at most $O(nn'^2)$.

The validity of Algorithm~\ref{alg:sparse-gaussian} is established in Theorem~\ref{thm:sg-ko} (proved in Appendix~\ref{app:thmsg-ko}).
%Theorem~\ref{thm:sg-ko} (proved in Appendix) shows Algorithm~\ref{alg:sparse-gaussian} outputs a valid knockoff.
\begin{theorem}\label{thm:sg-ko}
	For $\bX$ with rows $\bx_{i}^{\top}$ i.i.d. draws from the gaussian model~\eqref{eq:gauss_sparse}, Algorithm~\ref{alg:sparse-gaussian} produces valid knockoffs (that is, $\bXk$ drawn according to Algorithm~\ref{alg:sparse-gaussian} will satisfy Definition~\ref{def:cond-ko}).
\end{theorem}

%Note that since $I_j'$ contains an intersection with $\{1:j-1\}$, this constraint becomes increasingly hard to satisfy for increasing $j$, for instance, the first variable can have as many as $n-2$ neighbors, while the last variable can only have at most $(n-2)/2$. However, we can actually take advantage of the fact that SCIP is not variable-order-invariant and order the variables so that $|I_j|$ is non-increasing in $j$, which makes the sparsity condition on $E$ as weak as possible. 

Note that when $n\geq 1+ 2p$, one can always take $E$ to be $[p]\times[p]$, we are back to the setting of the previous section, and Algorithm~\ref{alg:sparse-gaussian} provides an alternative way to that in Theorem~\ref{thm:ldg_ko} for generating conditional knockoffs. 

\subsection{Proof of Theorem~\ref{thm:sg-ko} }\label{app:thmsg-ko}
For simplicity, we assume $\pi_j=j$ for all $j\in [p]$. In the process of Algorithm\ref{alg:sparse-gaussian}, the sets $N_j$ and $B$ are expanding. In this proof, $N_j$ refers to the set used in the $j$th step, after which the set remain unchanged; $B$ refers to the set after the final step.  For ease of notation, we use $\pr{\cdot}$ to denote the conditional probability given the sufficient statistics.   

Before getting into the detail of the proof, it is helpful to have an overview. In order to show the density function is invariant to swapping, we first find an explicit expression for the joint density of $(\bX,\bXk)$ in Lemma~\ref{lem:sparse-ggm-cond-density} and Conjecture~\ref{lem:gaussian-density}. This density function depends on the norms of residuals $\{\be_j\}_{j\in [p]}$ generated in the algorithm and a product of indicator functions. We  establish the swap-invariance of the product in Lemma~\ref{lem:sparse-ggm-set}  and Corollary~\ref{lem:gaussian-sym-set}, and the swap-invariance of  the norm of residuals in Lemma~\ref{lem:sparse-ggm-residual}. 

\begin{lemma}\label{lem:sparse-ggm-cond-density}
If $j\notin B$, then the $j$th step in Algorithm~\ref{alg:sparse-gaussian} draws $\bXk_j$ from the distribution:
\begin{align}\label{eq:scipj}
&\Pcr{\bXk_j =\bsfXk_j }{ \bX,\bXk_{1:(j-1)} } \nonumber \\
= \; &\frac{C_{d_j} }{\| \be_j\|^{d_j} } \one{ \bs{1}^{\top} \bsfXk_j =\bs{1}^{\top} \bX_j, \|\bsfXk_j \|=\|\bX_j \|} \prod_{k\in N_j }\one{\bX_k^{\top} \bsfXk_j =\bX_k^{\top} \bX_j } \prod_{k\in N_j^{-} }\one{\bXk_k^{\top} \bsfXk_j =\bXk_k^{\top} \bX_j },
\end{align}
where $d_j=n-(1+ |N_j|+|N_j^-|)$ and $C_{d_j}$ is a constant depending  only on $d_j$, and the base measure is the Hausdorff measure restricted on the set 
\begin{align*}
\begin{split}
\left\{ \bsfXk_j\in \R^{n}: \bs{1}^{\top} \bsfXk_j =\bs{1}^{\top} \bX_j, \, \|\bsfXk_j \|=\|\bX_j \|;  \right. \\
\left.  \forall k\in N_j ,\,  \bX_k^{\top} \bsfXk_j =\bX_k^{\top} \bX_j ; \right. \\
\left. \forall k\in N_j^{-},\, \bXk_k^{\top} \bsfXk_j =\bXk_k^{\top} \bX_j \right\}.
\end{split}
\end{align*}

If $j\in B$, then
\begin{align}\label{eq:scipjB}
\Pcr{\bXk_j =\bsfXk_j }{ \bX,\bXk_{1:(j-1)} } 
&=\one{\bsfXk_j=\bX_j}.
\end{align}

It follows that the density of $\bXk\mid \bX=\bsfX$ respective to the product of the above base measures is given by
\begin{align}\label{eq:scip-joint}
& \; \prod_{j \in B}\one{\bsfXk_j=\bX_j} \prod_{j\in [p]\setminus  B}\frac{C_{d_j} }{\| \be_j\|^{d_j} }\prod_{j\in [p]\setminus  B} \one{ \bs{1}^{\top} \bsfXk_j =\bs{1}^{\top} \bX_j , \|\bsfXk_j \|=\|\bX_j \|} \nonumber \\
& \times \prod_{j\in [p]\setminus  B}\left(  \prod_{k\in N_j }\one{\bX_k^{\top} \bsfXk_j =\bX_k^{\top} \bX_j } \prod_{k\in N_j^{-} }\one{\bsfXk_k^{\top} \bsfXk_j =\bsfXk_k^{\top} \bX_j } \right).
\end{align}
\end{lemma}

\begin{conjecture}\label{lem:gaussian-density}
Define 
\begin{align*}
M \; :=\;   \left\{ [\bsfX,\bsfXk]\in \R^{n\times 2p}  : \right.  &\left. \forall \; j \in B, \; \bsfXk_j=\bsfX_j; \; \forall \; j\in [p]\setminus  B, \; \bs{1}^{\top} \bsfXk_j =\bs{1}^{\top} \bsfX_j, \;  \|\bsfXk_j \|=\|\bsfX_j \| ,\right. \\
&\left. \forall \; k\in N_j, \; \bsfX_k^{\top} \bsfXk_j =\bsfX_k^{\top} \bsfX_j, \right. \\
&\left. \mbox{and } \forall \; k\in N_j^{-},  \; \bsfXk_k^{\top} \bsfXk_j =\bsfXk_k^{\top} \bsfX_j \right\}
\end{align*}

The joint density of $[\bX,\,\bXk]$ is 
\begin{align}
&\;  C_{0} \one{ \bs{1}^{\top}\bsfX_j =  \hat{\mu}_{j}, \forall \; j\in [p] } \one{ \bsfX_k^{\top}\bsfX_j=\hbS_{j,k}, \forall \; (j, k)\in E} \times \\
&\;  \one{[\bsfX,\bsfXk]\in M} \prod_{j\in [p]\setminus  B}\frac{C_{d_j} }{\| \be_j\|^{d_j} },\label{eq:sparse-ggm-sym}
\end{align}
where $C_{0}$ is a constant depending only on the sufficient statistics and the base measure is the Hausdorff measure restrict on the set 
\begin{align*}
\begin{split}
\left\{[\bsfX, \bsfXk]\in \R^{n\times(2p)}:  \bs{1}^{\top}\bsfX_j =  \hat{\mu}_{j}, \forall \; j\in [p] ; \bsfX_k^{\top}\bsfX_j=\hbS_{j,k}, \forall \; (j, k)\in E; [\bsfX,\bsfXk]\in M \right\} % \right. \\ \left. 
\end{split}
\end{align*}
\end{conjecture}

\begin{remark}
	Although it can be shown that the distribution of $\bX$ given the sufficient statistics is uniform on the set $\left\{\bsfX: T(\bsfX)=T(\bX) \right\}$, and it seems the conditional distribution given by Lemma~\ref{lem:sparse-ggm-cond-density} will show the joint distribution of $[ \bX,\bXk]$, we are not aware of any general result for probability measure on geometric sets that guarantees the expression of the joint density as the product of the marginal and the conditional. A special case where we can prove such a result is the Lemma~\ref{lem:ldg} in Section~\ref{app:ldgprf}. 
\end{remark}


\begin{lemma}\label{lem:sparse-ggm-set}
$M$ is invariant to swapping ,i.e., $[\bX,\,\bXk]_{\text{swap}(A)}\in M \iff [\bX,\,\bXk]\in M$, for any $A\subseteq [p]$. 
\end{lemma}

\begin{corollary}\label{lem:gaussian-sym-set}
	The set 
	\[
	\bar{M}=M\cap	\{[\bX,\bXk]\in \R^{n\times 2p} : \bs{1}^{\top}\bX_j =  \hat{\mu}_{j}, \forall \; j\in [p] , \bX_k^{\top}\bX_j=\hbS_{j,k}, \forall \; (j,k)\in E\}
	\]
	is also invariant to swapping.
\end{corollary}


Note that the length of the residual $\|\be_j\|$ created in the $j$th step is a function of $[\bX,\,\bXk]$. We can show it is also swap-invariant in our context. 
\begin{lemma}\label{lem:sparse-ggm-residual}
	For any $j\in [p]\setminus  B$, and any $A\subseteq [p]$, denote by $ \be_j^{A}$ the least-squares regression residual in the $j$th step with $[\bX,\,\bXk]$ replaced by $[\bX,\,\bXk]_{\text{swap}(A) }$.%, the matrix $\bX$ with the $k$th column replaced by $\bXk_k$ for $k\in A$. 
	Then $\| \be_j^{A}\|=\| \be_j\|$ if $[\bX,\bXk]\in M$. 
\end{lemma}


\begin{proof}[Proof of Theorem~\ref{thm:sg-ko} ]
	For any $A\subset [p]$, by Lemma~\ref{lem:sparse-ggm-set} and Corollary~\ref{lem:gaussian-sym-set}, swapping $\bX_A$ with $\bXk_A$ leaves the indicator functions in \eqref{eq:sparse-ggm-sym} unchanged. By Lemma~\ref {lem:sparse-ggm-residual}, $\| \be_j\|=\| \be_j^{A}\|$ for $[\bX,\bXk]\in M$.  Together with Corollary~\ref{lem:gaussian-density}, we conclude that
\[
\pr{ \bX,\bXk } =\pr{ [\bX,\bXk]_{\text{swap}(A) } } 
\]
\end{proof}

\subsection{Proofs of Preliminary Results}

\begin{proof}[Proof of Lemma~\ref{lem:sparse-ggm-cond-density}]% take from LJ's note
Equation~\eqref{eq:scipjB} is straightforward. Equation~\eqref{eq:scip-joint} follows from \eqref{eq:scipj} and \eqref{eq:scipjB} directly. We will prove \eqref{eq:scipj} in detail. 

%We prove by induction. 
Since the distribution in equation~\eqref{eq:scipj} is a product of indicator functions, it is simply the uniform distribution on the set on which those indicator functions are nonzero:
\begin{equation}
\begin{aligned}
%D_j&:=\left\{\bXk_j \in \R^{n} :\bXk_j^{\top}\bs{1}_n/n = \hmu_j,\; (\bXk_j-\hbmu_j)^\top(\bX_k-\hbmu_k)=\hbS_{j,k}\;\forall \; k\in N_j,\right.\\
%&\qquad\qquad \left.(\bXk_j-\hbmu_j)^\top(\bXk_k-\hbmu_k)=\hbS_{j,k}\;\forall \; k\in N_j^{-},\; \|\bXk_j-\hbmu_j\|^2 = \hbS_{j,j}\right\}
D_j&:=\left\{\bsfXk_j \in \R^{n} :\bsfXk_j^{\top}\bs{1}_n = \bX_j^{\top}\bs{1}_n ; \; \bsfXk_j^\top \bX_k=\bX_j^\top \bX_k,  \; \forall \; k\in N_j; \right.\\
&\qquad\qquad \left.  \bsfXk_j ^\top \bXk_k = \bsfX_j^\top \bX_k, \;\forall \; k\in N_j^{-} ; \; \|\bsfXk_j\| =\|\bX_j\|  \right\}.
\end{aligned}
\end{equation}

%Since $\bXk_{1:(j-1)}$ is sampled according to the algorithm, it holds that $\bXk_k^{\top}\bs{1}_n= \hmu_k $ holds for all $k<j$. Also note that $\bX$ yields the sufficient statistics,  $D_j$ can be written as
%\begin{equation}
%\begin{aligned}
%D_j&=\left\{\bXk_j \in \R^{n} :\bXk_j^{\top}\bs{1}_n/n = \hmu_j,\; (\bXk_j-\hbmu_j)^\top(\bX_k-\hbmu_k)=\hbS_{j,k}\;\forall \; k\in N_j,\right.\\
%&\qquad\qquad \left.(\bXk_j-\hbmu_j)^\top(\bXk_k-\hbmu_k)=\hbS_{j,k}\;\forall \; k\in N_j^{-},\; \|\bXk_j-\hbmu_j\|^2 = \hbS_{j,j}\right\}.
%\end{aligned}
%\end{equation}


Define 
\begin{equation}\label{eq:Dj}
\begin{aligned}
D'_j = \; &\left\{\hbmu_j + \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbsfe_j\,:\right.\\
& \qquad\left.\left[\bs{1}_n,\, \left(\bX_{N_j}-\hbmu_{N_j}\right),\, \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\right]^\top \tbsfe_j= \bs{0}_{|N_j|+|N_j^{-}|+1},\;\, \|\tbsfe_j\| = \|\be_j\|\right\} \\
= \; &\,\hbmu_j + \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} \\
&\qquad+\left\{\tbsfe_j \,:\;\left[\bs{1}_n,\, \left(\bX_{N_j}-\hbmu_{N_j}\right),\, \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\right]^\top\tbsfe_j= \bs{0}_{|N_j|+|N_j^{-}|+1},\;\, \|\tbsfe_j\| = \|\be_j\|\right\}
\end{aligned}
\end{equation}

We will show that $D_j=D'_{j}$. 
Once we have shown this, we will be done, since $\tbe_j$ is by definition drawn uniformly from the set defined by the last line of equation~\eqref{eq:Dj}, and thus since $\bXk_j$ is just a translation of $\tbe_j$, it is drawn uniformly from $D_j$. We now prove equation~\eqref{eq:Dj}:

Superset (``$\supseteq$"):
Suppose $\bsfXk_j\in D'_{j} $, we should show $ \bsfXk_j \in D_j$. First,

\begin{equation*}
\bsfXk_j^{\top}\bs{1}_n=\left(\hbmu_j + \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j'}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbsfe_j\right)^\top\bs{1}_n = \hbmu_j^\top\bs{1}_n = \bX_j^{\top}\bs{1}_n ,
\end{equation*}
because the columns of $\left(\bX_{N_j}-\hbmu_{N_j}\right)$ and $\big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)$ are all orthogonal to $\bs{1}_n$ by construction, and so is $\tbsfe_j$ by definition. \\

For any $k\in N_j$: 
\begin{equation}\label{eq:sup2}
\begin{aligned}
(\bsfXk_j-\hbmu_j)^\top(\bX_k-\hbmu_k)
&=\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbsfe_j\right)^\top(\bX_k-\hbmu_k) \\
&=\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j\right)^\top(\bX_k-\hbmu_k) \\
&=(\bX_j-\hbmu_j)^\top(\bX_k-\hbmu_k) ,
\end{aligned}
\end{equation}
where the second equality follows because $(\bX_k-\hbmu_k)^\top\tbsfe_j= 0 = (\bX_k-\hbmu_k)^\top\be_j$.Note that 
\[
\hbmu_j^\top(\bX_k-\hbmu_k)=0,
\] and \[\bsfXk_j ^{\top} \hbmu_k = \hmu_k \bsfXk_j ^{\top}\bs{1}_{n}=\hmu_k \bX_j ^{\top}\bs{1}_{n}=\bX_j ^{\top} \hbmu_k,\]  we conclude $\bsfXk_j^\top\bX_k=\bX_j^\top\bX_k$. 


For any $k\in N_j^{-}$:
\begin{equation}\label{eq:sup3}
\begin{aligned}
(\bsfXk_j-\hbmu_j)^\top(\bXk_k-\hbmu_k)
&=\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbsfe_j\right)^\top(\bXk_k-\hbmu_k) \\
&=\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j\right)^\top(\bXk_k-\hbmu_k) \\
&=(\bX_j-\hbmu_j)^\top(\bXk_k-\hbmu_k) ,
\end{aligned}
\end{equation}
where again the second equality follows because $(\bXk_k-\hbmu_k)^\top\tbsfe_j= 0 = (\bXk_k-\hbmu_k)^\top\be_j$, and we conclude 
\[
\bsfXk_j^\top\bXk_k = \bX_j^\top\bXk_k.
\]

Finally, checking the last condition in $D_j$:
\begin{equation*}\label{eq:sup4}
\begin{aligned}
&\qquad \|\bsfXk_j\|^2 - n \hmu_j^{2}\\
&=\; (\bsfXk_j-\hbmu_j)^\top(\bsfXk_j-\hbmu_j)  \\
&=\;\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbsfe_j\right)^\top\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \tbsfe_j\right) \\
&=\; \|\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\|^2 + \|\tbsfe_j\|^2 \\
&=\; \|\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\|^2 + \|\be_j\|^2 \\
&=\; \left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j\right)^\top\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j\right) \\
&=\; (\bX_j-\hbmu_j)^\top(\bX_j-\hbmu_j)\\
&=\; \|\bX_j\|^2 - n \hmu_j^{2},
\end{aligned}
\end{equation*}
where the third and fifth equalities follows because $\left[\left(\bX_{N_j}-\hbmu_{N_j}\right),\, \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\right]^\top\tbsfe_j= \bs{0}_{|N_j|+|N_j^{-}|} = \left[\left(\bX_{N_j}-\hbmu_{N_j}\right),\, \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\right]^\top\be_j$, so all the cross terms cancel in the quadratic expansion. The fourth equality follows from the constraint that $\|\tbsfe_j\| = \|\be_j\|$. This proves the superset property.\medskip

Subset (``$\subseteq$"): Suppose $\bsfXk_j\in D_j$, we should show $\bsfXk_j\in D'_{j}$. \\
Define $\tbsfe_j=\bsfXk_j-\hbmu_j - \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} - \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}$, 
\begin{equation*}
\bs{1}_n^\top \tbsfe_j= \bs{1}_n^\top\left(\bsfXk_j-\hbmu_j - \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} - \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\right) = \bs{1}_n^\top \bsfXk_j-\bs{1}_n^\top\bX_j = 0,
\end{equation*}
where the second equality uses the fact that  $\bs{1}_n^\top\left(\bX_{N_j}-\hbmu_{N_j}\right) = \bs{0}$ and $ \bs{1}_n^\top\bXk_{N_j^{-}}=\bs{1}_n^\top \bX_{N_j^{-}}$. 

Next for any $k\in N_j$,
\begin{equation*}
\begin{aligned}
\left(\bX_k-\hbmu_k\right)^\top\tbsfe_j&=\; \left(\bX_k-\hbmu_k\right)^\top\left(\big(\bsfXk_j-\hbmu_j\big) - \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} - \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\right) \\
&= \; \left(\bX_k-\hbmu_k\right)^\top\big(\bsfXk_j-\hbmu_j\big)  - \left(\bX_k-\hbmu_k\right)^\top\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j\right) \\
&= \; \left(\bX_k-\hbmu_k\right)^\top\big(\bsfXk_j-\hbmu_j\big)   - \left(\bX_k-\hbmu_k\right)^\top\left(\bX_j-\hbmu_j\right) \\
&=\;  \bX_k^\top\bsfXk_j-\bX_k^\top\bX_j=0,
\end{aligned}
\end{equation*}
where the second equality follows from the facts that $\left(\bX_k-\hbmu_k\right)^\top\be_j = 0$ and the fourth equality use $\hbmu_k^\top\bsfXk_j=\hbmu_k^\top\bsfXk_j$. 

Next for $k\in N_j^{-}$,
\begin{equation*}
\begin{aligned}
\big(\bXk_k-\hbmu_k\big)^\top\tbsfe_j&= \big(\bXk_k-\hbmu_k\big)^\top\left(\big(\bsfXk_j-\hbmu_j\big) - \left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} - \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\right) \\
&= \; \big(\bXk_k-\hbmu_k\big)^\top\big(\bsfXk_j-\hbmu_j\big)  - \big(\bXk_k-\hbmu_k\big)^\top\left(\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} + \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)} + \be_j\right) \\
&= \; \big(\bXk_k-\hbmu_k\big)^\top\big(\bsfXk_j-\hbmu_j\big)   - \big(\bXk_k-\hbmu_k\big)^\top\left(\bX_j-\hbmu_j\right) \\
&=\; \bXk_k^\top\bsfXk_j-\bXk_k^\top\bX_j = 0,
\end{aligned}
\end{equation*}
where similarly the second equality follows from the facts that $\big(\bXk_k-\hbmu_k\big)^\top\be_j = 0$, and the fourth equality follows from $\hbmu_k^\top\bsfXk_j=\hbmu_k^\top\bsfXk_j$. 

And finally,
\begin{equation*}
\begin{aligned}
\| \tbsfe_j\|^2 &= \left\|\bsfXk_j-\hbmu_j\right\|^2 - \left\|\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} - \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\right\|^2 \\
&= \left\|\bX_j-\hbmu_j\right\|^2 - \left\|\left(\bX_{N_j}-\hbmu_{N_j}\right)\hbb^{(j)} - \big(\bXk_{N_j^{-}}-\hbmu_{N_j^{-}}\big)\tbb^{(j)}\right\|^2 \\
&= \|\be_j\|^2,
\end{aligned}
\end{equation*}
where the first and third equalities follow from the Pythagorean theorem, and the second follows from the fact that 
\[
\left\|\bsfXk_j-\hbmu_j\right\|^2 = \left\| \bsfXk_j \right\| ^{2} + \left\|\hbmu_j\right\|^2 - 2 \bsfXk_j^{\top }\bs{1}_{n} \hmu_j= \left\| \bX_j   \right\|^{2} + \left\|\hbmu_j\right\|^2 - 2 \bX_j^{\top }\bs{1}_{n} \hmu_j = \left\|\bX_j-\hbmu_j\right\|^2.\] 
This proves the subset property, and thus the two sets are equal and the lemma is proved.
\end{proof}


Before showing the product of indicator functions is invariant to swapping, we prove the following lemma. 
\begin{lemma}\label{lem:sp-gaussian-include}
For any $k\in [p]\setminus  B$, and any $ j \in N_k^{+}$, it holds that 
\begin{enumerate}
	\item[(a).] $N_k\setminus  \{j\}\subseteq N_j$
	\item[(b).]  $k\in N_j^{-}$. 
%	\item $\bXk_{j}^{\top}\bX$
\end{enumerate}
\end{lemma}
\begin{proof}
(a) follows from the $k$th update step in the algorithm. 	\\
If $(j,k) \in E$, (b) holds. Otherwise, there is some $l<k$, such that $k,j\in N_l^{+}$, and it follows that $k\in N_j$ by the $l$th update step. Since $k<j$ and $k\notin B$, we conclude that $k\in N_j^-$. 
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:sparse-ggm-set}]
%	Assume $[\bX,\,\bXk]\in M$. For $A=\{j\}$, we check if the conditions involving $ \bXk_j$ and  $\bX_j$ is invariant to swapping these two. If $j \in B$, $\bXk_j=\bX_j$ so it is true. If $j\notin B$, 
%	\begin{enumerate}[(a).]
%		\item When $j$ is the same as the $j$ as in the definition of set $M$:
%	\[\bs{1}^{\top} \bXk_j =\bs{1}^{\top} \bX_j, \; \|\bXk_j \|=\|\bX_j \|; \; \forall \; k\in N_j, \; \bX_k^{\top} \bXk_j =\bX_k^{\top} \bX_j ;\; \forall \; k\in N_j^{-},  \; \bXk_k^{\top} \bXk_j =\bXk_k^{\top} \bX_j \]
%	 are invariant to swapping $ \bXk_j$ and  $\bX_j$. 
%\item When $j$ appears as the $k\in N_j^{-}$ in the second and third lines in the definition of $M$: suppose $k\notin B$ such that $j\in N_k^{-}$, the equations in the second and third lines are
%	\[ \bX_j^{\top} \bXk_i =\bX_j^{\top} \bX_i, \quad  \bXk_j^{\top} \bXk_i =\bXk_j^{\top} \bX_i\]
%	 is invariant to  swapping $ \bXk_j$ and  $\bX_j$. 
%\item When $j$ appears as the $k$ in the second line in the definition of $M$: suppose $k\notin B$ such that $j\in N_k^{+}$,  the equation in the second line is $\bX_j^{\top} \bXk_k=\bX_j^{\top} \bX_k  $. By Lemma~\ref{lem:sp-gaussian-include}(b), $k\in N_j^{-}$ , and the second and third lines of the definition implies
%$\bX_k^{\top} \bXk_j =\bX_k^{\top} \bX_j,  \bXk_k^{\top} \bXk_j =\bXk_k^{\top} \bX_j $.  Hence all these four quantities are equal and 
%\[ \bXk_j^{\top} \bXk_k=\bXk_j^{\top} \bX_k. \] 
%	
%	\end{enumerate}
%This shows $[\bX,\,\bXk]_{\text{swap}(\{j\}) }\in M$. For general $A$, apply the same arguments to each element one by one and we conclude $[\bX,\,\bXk]_{\text{swap}(A) }\in M$.\\
%The opposite direction follows by swapping twice. 
%\end{proof}
	Assume $[\bX,\,\bXk]\in M$. For $A=\{a\}$, we check if the conditions involving $ \bXk_a$ and  $\bX_a$ is invariant to swapping these two. If $a \in B$, $\bXk_a=\bX_a$ so it is true. If $a\notin B$, 
	\begin{enumerate}[(a).]
		\item When $a$ appears as $j$ in the definition of $M$:
	\begin{align*}
 \bs{1}^{\top} \bXk_a =\bs{1}^{\top} \bX_a, \; \|\bXk_a \|=\|\bX_a \|; \; \forall \; k\in N_a, \; \bX_k^{\top} \bXk_a =\bX_k^{\top} \bX_a ;\\
  \forall \; k\in N_a^{-},  \; \bXk_k^{\top} \bXk_a =\bXk_k^{\top} \bX_a 
	\end{align*}
	 are invariant to swapping $ \bXk_a$ and  $\bX_a$. 
\item When $a$ appears as the $k\in N_j^{-}$ in the second and third lines of the definition of $M$: suppose $j\notin B$ such that $a\in N_j^{-}$, the equations in the second and third lines 
	\[ \bX_a^{\top} \bXk_j =\bX_a^{\top} \bX_j, \quad  \bXk_a^{\top} \bXk_j =\bXk_a^{\top} \bX_j\]
	are  invariant to  swapping $ \bXk_a$ and  $\bX_a$. 
\item When $a$ appears as the $k\in N_j^{+}$ in the second line of the definition of $M$: suppose $j\notin B$ such that $a\in N_j^{+}$,  the equation in the second line is $\bX_a^{\top} \bXk_j=\bX_a^{\top} \bX_j  $. We will show this equation still holds when swapping $ \bXk_a$ and  $\bX_a$. \\
By Lemma~\ref{lem:sp-gaussian-include}(b), $j\in N_a^{-}$ , and the second and third lines of the definition implies
$\bX_j^{\top} \bXk_a =\bX_j^{\top} \bX_a,  \bXk_j^{\top} \bXk_a =\bXk_j^{\top} \bX_a $.  Hence all these four quantities are equal and 
\[ \bXk_a^{\top} \bXk_j=\bXk_a^{\top} \bX_j, \] 
	that is, the equation in this case is invariant to swapping. 
	\end{enumerate}
This shows $[\bX,\,\bXk]_{\text{swap}(\{a\}) }\in M$. For general $A$, apply the same arguments to each element one by one and we conclude $[\bX,\,\bXk]_{\text{swap}(A) }\in M$.\\
The opposite implication follows by swapping twice. 
\end{proof}

\begin{proof}[Proof of Corollary~\ref{lem:gaussian-sym-set}]
 	Assume $[\bX,\,\bXk]\in \bar{M}$. Suppose $A=\{j\}$, we will show $[\bX,\,\bXk]_{\text{swap}(\{j\}) }\in \bar{M}$. The remaining argument is the same as the proof of Lemma~\ref{lem:sparse-ggm-set}. 
 	
 	Since Lemma~\ref{lem:sparse-ggm-set} implies $[\bX,\,\bXk]_{\text{swap}(\{j\}) }\in M$, we only need to show $\bs{1}^{\top}\bX_j =  \hat{\mu}_{j}$ and $\bX_k^{\top}\bX_j=\hat{\Sigma}_{j,k}, \forall \; (j,k)\in E$ also hold for replacing $\bX_j$ by $\bXk_j$. If $j\in B$, then $\bXk_j=\bX_j$ and it is done. 
 	
Suppose $j\notin B$.  	From the definition of $M$, we have $\bs{1}^{\top}\bXk_j =\bs{1}^{\top}\bX_j = \hat{\mu}_{j}$ .  For any $(j,k)\in E$, the third line of the definition of $M$ reads $\bX_k^{\top} \bXk_j=\bX_k^{\top}\bX_j=\hat{\Sigma}_{j,k}$. We conclude that $[\bX,\,\bXk]_{\text{swap}(\{j\}) }\in \bar{M}$. 
%If $j\in B$ it follows from part (b) in the proof of Lemma~\ref{lem:sparse-ggm-set}. If $k\in B$, it follows from part (b) in the proof of Lemma~\ref{lem:sparse-ggm-set}. If $j,k\notin B$, note $k\in N_j^+$, it follows from part (c) in the proof of Lemma~\ref{lem:sparse-ggm-set}.

\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:sparse-ggm-residual}]
Define $\bs{U}=	\left[\bs{1}_n,\, \left(\bX_{N_j^{-}}-\hbmu_{N_j^{-}}\right),\, \left( \bXk_{N_j^{-}}-\hbmu_{N_j^{-}} \right), \left(\bX_{N_j^{+}}-\hbmu_{N_j^{+}}\right) \right]$. 
Because $\| \be_j\|^{2}=\|\bX_j\|^{2}- \bX_j^{\top}\bs{U} (\bs{U}^{\top}\bs{U})^{-1} \bs{U}^{\top} \bX_j$ and the definition of $M$ implies $\|\bX_j\|=\|\bXk_j\|$, we only need to show  $\bX_j^{\top}\bs{U} (\bs{U}^{\top}\bs{U})^{-1} \bs{U}^{\top} \bX_j$  is invariant to swapping. 

By the symmetry of $\bX_{N_j^{-}}$ and $\bXk_{N_j^{-}}$ in $\bs{U}(\bs{U}^{\top}\bs{U})^{-1}\bs{U}^{\top}$, we can assume $N_j^{-}\cap A =\emptyset$.  
\begin{enumerate}[(a).]  
	\item Show $\bU\tp \bX_j$ is swap-invariant. It follows from the definition of $M$ that
\begin{align}
\label{eq:lem-sparse-ggm-swap-ux1}
\left(\bs{1}_n, \bX_{N_j^{-}}, \bXk_{N_j^{-}}, \bX_{N_j^{+}} \right) ^{\top} \bX_j=\left(\bs{1}_n, \bX_{N_j^{-}}, \bXk_{N_j^{-}}, \bX_{N_j^{+}} \right) ^{\top} \bXk_j,
\end{align}
Since $\hbmu_{l}=\hmu_{l}\bs{1}_{n}$, \eqref{eq:lem-sparse-ggm-swap-ux1} implies 
\begin{align*}
\left(\bs{1}_n, \bX_{N_j^{-}}-\hbmu_{N_j^{-}}, \bXk_{N_j^{-}}-\hbmu_{N_j^{-}}, \bX_{N_j^{+}}-\hbmu_{N_j^{+}} \right) ^{\top} \bX_j\\
=\left(\bs{1}_n, \bX_{N_j^{-}}-\hbmu_{N_j^{-}}, \bXk_{N_j^{-}}-\hbmu_{N_j^{-}}, \bX_{N_j^{+}}-\hbmu_{N_j^{+}} \right)  ^{\top} \bXk_j,
\end{align*}
which shows $\bU\bX_j$ is unchanged when swapping $\bX_j$ and $\bXk_j$. Part (c) of the proof of  Lemma~\ref{lem:sparse-ggm-set} implies
\begin{align}
\label{eq:lem-sparse-ggm-swap-ux2}
\bX_{N_j^{+}} ^{\top} \bX_j=\bXk_{N_j^{+} } ^{\top} \bX_j, \text{ and } \bXk_{N_j^{+} }^{\top} \bX_j=\bXk_{N_j^{+}}  ^{\top} \bXk_j, 
\end{align}
thus $\bX_{N_j^{+} } ^{\top} \bXk_j =\bX_{N_j^{+}} ^{\top} \bX_j= \bXk_{N_j^{+} }^{\top} \bX_j=\bXk_{N_j^{+}}  ^{\top} \bXk_j$.  We conclude that $\bs{U}\bX_j$  is invariant to swapping $A$. \\
\item 
To show $(\bs{U}^{\top}\bs{U})$ is swap-invariant, we swap the elements in $A\cap N_j^+$ one by one from the largest to the smallest. \\
By Lemma~\ref{lem:sp-gaussian-include}(a), for any $k\in N_j^{+}$, $N_j\setminus  \{k\}\subseteq N_k$, similar to part (a), it holds that
\begin{align}
\label{eq:lem-sparse-ggm-swap-uu1}
\left( \bX_{N_j^{-}}, \bXk_{N_j^{-}}, \bX_{N_j^{+}\setminus  k},\bXk_{N_j^{+}\setminus  k } \right) ^{\top} \bX_k=\left( \bX_{N_j^{-}}, \bXk_{N_j^{-}}, \bX_{N_j^{+}\setminus  k}, \bXk_{N_j^{+}\setminus  k}  \right) ^{\top} \bXk_k,
\end{align}
and
\begin{align}
\label{eq:lem-sparse-ggm-swap-uu2}
\bX_{N_j^{+}\cap N_k^{+} } ^{\top} \bXk_k=\bX_{N_j^{+}\cap N_k^{+}} ^{\top} \bX_k=\bXk_{N_j^{+}\cap N_k^{+} } ^{\top} \bX_k=\bX_{N_j^{+}\cap N_k^{+}} ^{\top} \bXk_k. 
\end{align}
Equation~\eqref{eq:lem-sparse-ggm-swap-uu1} implies $(\bs{U}^{\top}\bs{U})$ is unchanged when swapping the largest $k_{(1)}\in A\cap N_j^+$. After this swap, Equation~\eqref{eq:lem-sparse-ggm-swap-uu1} together with Equation~\eqref{eq:lem-sparse-ggm-swap-uu2} guarantees $(\bs{U}^{\top}\bs{U})$ is unchanged when swapping the second largest $k_{(2)}\in A\cap N_j^+$. The same argument applies to each $k$ in $A\cap N_j^+$ after swapping those larger than $k$. We conclude that $(\bs{U}^{\top}\bs{U})$ is swap-invariant. 
\end{enumerate}
\end{proof}



